No-Regret Exploration in Goal-Oriented Reinforcement Learning

Many popular reinforcement learning problems (e.g., navigation in a maze, some Atari games, mountain car) are instances of the episodic setting under its stochastic shortest path (SSP) formulation, where an agent has to achieve a goal state while minimizing the cumulative cost. Despite the popularity of this setting, the exploration-exploitation dilemma has been sparsely studied in general SSP problems, with most of the theoretical literature focusing on different problems (i.e., fixed-horizon and infinite-horizon) or making the restrictive loop-free SSP assumption (i.e., no state can be visited twice during an episode). In this paper, we study the general SSP problem with no assumption on its dynamics (some policies may actually never reach the goal). We introduce UC-SSP, the first no-regret algorithm in this setting, and prove a regret bound scaling as $\displaystyle \widetilde{\mathcal{O}}( D S \sqrt{ A D K})$ after $K$ episodes for any unknown SSP with $S$ states, $A$ actions, positive costs and SSP-diameter $D$, defined as the smallest expected hitting time from any starting state to the goal. We achieve this result by crafting a novel stopping rule, such that UC-SSP may interrupt the current policy if it is taking too long to achieve the goal and switch to alternative policies that are designed to rapidly terminate the episode.

==> app_experiments.tex <==
% !TEX root = SSP_paper.tex

\section{Experiments}
\label{app:experiments}

\begin{figure}[t]
        \centering
            % \includegraphics[width=.32\textwidth]{./exp/gridworld_uniform_costs/regret_episodes.pdf}\hfill
            % \includegraphics[width=.32\textwidth]{./exp/gridworld_uniform_costs/regret_time.pdf}\hfill
            % \includegraphics[width=.32\textwidth]{./exp/gridworld_uniform_costs/avglength_episodes.pdf}

        \includegraphics[width=.38\textwidth]{./exp/UNSMALL/regret_episodes.pdf} \tikz[remember picture, baseline]{\node (aa) at (0,0) {};}
        \hspace{1.4in}
        \includegraphics[width=.37\textwidth]{./exp/UNSMALL/regret_time.pdf}\\
        \hspace*{.1in}\includegraphics[width=.37\textwidth]{./exp/UNSMALL/avglength_episodes.pdf}\hspace{1.4in}
        \includegraphics[width=.36\textwidth]{./exp/UNSMALL/UCSSP-H_avgest_hittingtime.pdf}

        \caption{Comparison of \UCSSP and \UCRL in the case of uniform-cost SSP. The plots are averaged over $200$ repetitions. We report the mean and the maximum and minimum value for top line and figure bottom right. For the bottom-left figure, we report the standard deviation of the mean at 96\% to simplify the visualization.}
        \label{fig:gridworld.uniform}
\end{figure}


In this section, we empirically validate our theoretical findings and perform an ablation study of the algorithms.
We consider $3$ scenarios: 1) uniform-cost SSP; 2) SSP with $c_{\min} > 0$ and 3) SSP with $c_{\min} = 0$.
In all the experiments, we consider the same $(3 \times 4)$ gridworld but we modify the cost function.
The agent can move using the cardinal actions (Right, Down, Left, Up).
An action fails with probability $p_{f} = 0.05$. In this case (failure), the agent uniformly follows one of the other directions.
Walls are absorbing, i.e., if the action leads against the wall, the agent stays in the current position with probability 1. For example, $p((0,0) | (0,0), right) = \frac{2p_{f}}{3}$, $p((1,0) | (0,0), right) = \frac{p_{f}}{3}$ and $p((0,1) | (0,0), right) = 1 - p_{f}$.
If we consider \emph{Up}, we have $p((0,0)|(0,0), Up) = 1$.
%\todoj{Not sure to understand this.}
For the experiments we used the theoretical confidence intervals without constants, i.e., $\beta_{k,j}(s,a) = \sqrt{\frac{S L}{N^+_{k,j}(s,a)}}$ with $L = \log(SAN^+_{k,j}(s,a)/0.1)$.%\todojout{I removed the $S$ in the log term}\todomout{I have it in the code. I don't want to rerun it now :) }
The remaining parameters are set as prescribed by the theory.
All the results are averaged over $200$ runs.

1) The first experiment aims to compare \UCRLtwo \citep{jaksch2010near} and \UCSSP in the case of uniform-cost SSP studied in Sect.\,\ref{section_uniform_costs} (see Fig.\,\ref{fig:gridworld.uniform}).
Thus we set $c(s,a) = 1$ for any $(s,a) \in \mathcal{S} \times \mathcal{A}$, and $c(\wb s,a) =0$ for all $a \in \mathcal{A}$.
We evaluate the algorithms at $K=3000$ episodes.
Fig.\,\ref{fig:gridworld.uniform}(top left) shows that the regret of both algorithms is sublinear, as stated by the theoretical analysis. Interestingly, the regret of \UCRL is higher than the one incurred by \UCSSP.
This is possibly due to algorithmic structure of \UCRL, which behaves in epochs (or algorithmic episodes) and each epoch ends when the number of visits to some state-action pair is doubled. \UCRL computes the policy only at the beginning of an epoch. As shown by the vertical lines in Fig.\,\ref{fig:gridworld.uniform}(top left), between each planning step, the agent may reach the goal multiple times.
While this can be computationally efficient, the drawback is that \UCRL may execute sub-optimal policies for long time.
On the other hand, we believe that by planning more often, \UCSSP is able to execute better policies than \UCRL. In fact, Fig.\,\ref{fig:gridworld.uniform}(bottom left) shows that the time required by \UCRL to reach the goal $\wb s$ is often higher than the one of \UCSSP.
It also shows that the length of phase \ding{173} in \UCSSP quickly goes to zero, meaning that policy executed by \UCSSP is able to quickly reach the goal.
Fig.\,\ref{fig:gridworld.uniform}(top right) shows that \UCRL requires more time (i.e., steps) than \UCSSP to successfully complete $2000$ episodes.
This test sheds light on the relationship between \UCRL and \UCSSP and shows that, despite the good regret guarantees, \UCRL may not exploit the specific structure of the SSP problem and poorly performs compared to \UCSSP.
Finally, we also plot the estimate of the hitting time computed by \UCSSP (see Fig.\,\ref{fig:gridworld.uniform}(bottom right)). As expected, it is a ``tight'' upper-bound to the expected hitting time of the optimal SSP policy ($\mathbb{E}[\tau_{\pi^\star}(s_0)] = 5.3$), except in the initial episodes where the optimistic model is far away from the true one. In the latter case, the imagined SSP problem has high probability of reaching $\wb s$ from any other state due to the high uncertainty.

\begin{tikzpicture}[remember picture,overlay]
  \node[anchor=west] at ($(aa)+(-.1in,0)$) {\includegraphics[width=4cm]{./exp/grid_1}};
  % \draw (current page.center) circle (3cm);
\end{tikzpicture}

\begin{figure}[bt]
  \centering
  \begin{minipage}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./exp/grid_2}
  \end{minipage}
  \begin{minipage}{.65\textwidth}
    \centering
    % \includegraphics[width=.8\textwidth]{./exp/gridworld_standard/regret_episodes}
    \includegraphics[width=.8\textwidth]{./exp/POSSMALL/regret_episodes}
  \end{minipage}
  \caption{Evaluation of the effect of $c_{\min} > 0$ on the regret of \UCSSP. Results are averaged over $200$ runs. We report mean value and maximum and minimum observed values.}
  \label{fig:gridworld.standard}
\end{figure}


\begin{figure}[tb]
  \centering
 % \begin{minipage}{.3\textwidth}
 %   \centering
 %   \includegraphics[width=\textwidth]{./exp/grid_3}
 % \end{minipage}
 % \begin{minipage}{.65\textwidth}
 %   \centering
 %   \includegraphics[width=.8\textwidth]{./exp/gridworld_zero_0.4/regret_episodes.png}
 % \end{minipage}
            \includegraphics[width=.32\textwidth]{./exp/grid_3}\hspace{1in}
            \includegraphics[width=.4\textwidth]{./exp/ZSMALL2/regret_episodes.pdf}\\
            \includegraphics[width=.4\textwidth]{./exp/ZSMALL2/avglength_episodes.pdf}\hspace{1in}
            \includegraphics[width=.4\textwidth]{./exp/ZSMALL2/UCSSP-H_avgest_hittingtime.pdf}
            \caption{Evaluation of \UCSSP for $c_{\min} = 0$. See Fig.\,\ref{fig:gridworld.uniform} for details.}
  \label{fig:gridworld.zero}
\end{figure}

2) The second experiment focuses on non-uniform cost. At each step, the agent incurs a cost of $\beta>0$ except when in $\wt{s}=(1,1) = P$ where the cost is $1$. The state $\wt{s}$ is considered to be a sand pit and has the effect of slowing down the agent (i.e., higher cost). Formally, $c(s,a) =\beta$ for all $(s,a) \in (\mathcal{S}\setminus\{\wt s\}) \times \mathcal{A}$, $c(\wt s, a) = 1$ for all $a \in \mathcal{A}$, and $c(\wb s,a) =0$ for all $a \in \mathcal{A}$. Clearly, $c_{\min} = \beta > 0$.
Note that the optimal SSP policy is the same for all the selected values of $\beta$.
As before, we evaluate the algorithms at $K=3000$ episodes.
In Fig.\,\ref{fig:gridworld.standard}(right) we show the impact of $c_{\min}$ on the regret of \UCSSP.
First of all, we show how $c_{\min}$ affects the true solution of the SSP problem. To do so, we run VI on the true model with $\epsilon=1.e-10$ and obtain
\[
V^\star(s_0|\beta=0.5) = 2.66,~~
V^\star(s_0|\beta=0.1) = 0.55,~~
V^\star(s_0|\beta=0.01) = 0.07,~~
V^\star(s_0|\beta=0.001) = 0.02.
\]
To remove the impact of the different magnitude of the cost, we consider the normalized regret $\wb \Delta(\mathfrak{A}, K) := \frac{\Delta(\mathfrak{A}, K)}{V^\star(s_0)}$.
Fig.\,\ref{fig:gridworld.standard}(right) shows that the complexity of the learning problem is proportional to $1/c_{\min}$, in the sense that the smaller $c_{\min}$ the higher the regret (i.e., the higher the learning complexity). This supports our theoretical result.



3) The final experiment deals with the case $c_{\min} = 0$.
We consider the states $(0,0), (0,1), (1,1)$ and $(1,0)$ to have zero cost, see Fig.\,\ref{fig:gridworld.zero}(left).
All the other states have cost defined as in experiment 2) with $\beta=0.4$. 
Note that there exists loops with zero costs, which means that there exist improper policies with finite $V$-values.
As mentioned in App.\,\ref{subsection_relaxation_asm_positive_costs}, in this case we compete against the optimal proper policy (see Fig.\,\ref{fig:gridworld.zero}(top left)).
To compute the optimal proper policy and its value $V$, we use VI with perturbation of $1e-10$~\citep{bertsekas2013stochastic}.
We evaluate the algorithms at $K=3000$ episodes.
We notice that \UCSSP has sublinear regret as expected. The perturbation of the costs has a large impact on the initial phase of \UCSSP when both uncertainty and perturbation are high. In this case, \UCSSP highly overestimates the hitting time of the optimal policy, leading to the execution of suboptimal policies for a long time (due to Phase \ding{172}). Once the perturbation and/or the uncertainty decreases, we notice that the estimated hitting time drops rapidly and approaches the true value.
It is also interesting to notice that the estimated hitting time of phase \ding{173} is never too high. This is due to the fact that phase \ding{173} aims to find the policy reaching the goal state in the smallest time.




\subsection{Bernstein Inequalities}
In this section, we provide an evaluation of the proposed algorithm with Bernstein inequalities and perform empirical comparison with later work \citep{cohen2020near}. 
Similarly to~\citep[e.g.,][]{azar2017minimax,improved_analysis_UCRL2B}, we consider the following concentration inequality of the transition probabilities: $\forall (s,a,s') \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}'$,
\begin{equation}
  \left| \wt{p}(s'|s,a) - \wh p_{k,j}(s'|s,a) \right| \leq \beta_{k,j}(s,a,s') \approx \sqrt{\frac{\sigma_p^2(s,a,s') L}{N^+_{k,j}(s,a)}} + \frac{L}{N^+_{k,j}(s,a)}
\end{equation}
where $L = \log(SAN^+_{k,j}(s,a)/0.1)$ and $\sigma_p^2(s,a,s') = \wh{p}_{k,j}(s'|s,a) (1 - \wh p_{k,j}(s'|s,a))$.

SSP planning can be performed using two approaches: \textcircled{a} extended value iteration (as in Alg.\,\ref{algorithm_VI_SSP}); \textcircled{b} computing an optimistic transition kernel $\wt{p}$ and planning via standard SSP value iteration~\citep[as in][]{cohen2020near}.
When planning with \emph{extended value iteration} (case \textcircled{a}) we use the optimistic Bellman operator defined in Eq.\,\eqref{eq_bellman_operator} with $B_{k,j}(s,a) := \{ \widetilde{p} \in \mathcal{C} ~\vert ~ \widetilde{p}(\cdot \, \vert \,  \overline{s},a) = \mathds{1}_{\overline{s}}, |\widetilde{p}(s' \, \vert \,  s,a) - \widehat{p}_{k,j}(s' \, \vert \,  s,a)| \leq \beta_{k,j}(s,a,s')\}$.
%
In case \textcircled{b}, we follow the approach in~\citep{cohen2020near}. We compute an optimistic transition kernel $\wt{p}_{k,j}$ defined as
\begin{align}
  \forall(s,a,s')\in \mathcal{S} \times \mathcal{A} \times \mathcal{S}, \hspace{.5in}&\wt{p}_{k,j}(s'|s,a) = \max \big\{0, \wh{p}_{k,j}(s'|s,a) - \beta_{k,j}(s,a,s')  \big\}\\
  \forall  (s,a) \in \mathcal{S} \times \mathcal{A},\hspace{.5in} & \wt{p}_{k,j}(\wb s|s,a) = 1 - \sum_{s' \in \mathcal{S}} \wt{p}_{k,j}(s'|s,a)
\end{align}
and solve the associated SSP problem using value iteration.
This guarantees optimism since $\wt{p}_{k,j}(s'|s,a) \leq p(s'|s,a)$ for  all transitions to non-goal states and $\wt{p}_{k,j}(\wb s|s,a) \geq p(\wb s|s,a)$.
Note that $\wt p_{k,j}(\cdot|s,a)$ may not belong to $B_p(s,a)$ since $\wt p_{k,j}(\wb s| s,a)$ may not satisfy the concentration inequality $|\wt p_{k,j}(\wb s| s,a) - \wh p_{k,j}(\wb s| s,a)| \leq \beta(s,a,\wb s)$.
Given the mentioned construction we have that $|\wt p_{k,j}(\wb s| s,a) - \wh p_{k,j}(\wb s| s,a)| \leq \sum_{s' \in \mathcal{S}} \beta(s,a,s')$.

\begin{figure}[bt]
  \centering
  \includegraphics[width=.48\textwidth]{./exp/bernstein/uniform/1/regret_episodes.pdf}
  \hfill
  \includegraphics[width=.48\textwidth]{./exp/bernstein/uniform/2/regret_episodes.pdf}
  \caption{Evaluation of the algorithms with Bernstein inequalities and uniform cost. See Fig.\,\ref{fig:gridworld.uniform} for details. We average the results over $200$ runs and report the standard deviation of the mean at 96\%. For clarity, we report the planning technique used for each algorithm. We recall that \textcircled{a} stands for \EVI\ while \textcircled{b} stands for the two-step procedure (computing $\wt p$ and planning through value iteration). We use \textcolor{gray}{(orig.)} to denote the algorithm as described in the original paper.}
\label{fig:bernstein.uniform}
\end{figure}

We compare  with \UCRLSSP~\citep{cohen2020near}. \UCRLSSP is a variant of \UCRLB~\citep{improved_analysis_UCRL2B} where the average reward planning is replaced with the SSP planning. In the original paper, \UCRLSSP uses the SSP planning defined in case~$\textcircled{b}$. Here, we run the algorithm with both planning approaches. When $c_{\min} = 0$, \UCRLSSP leverages the same perturbation idea used by \UCSSP. The cost is then defined as $c(s,a) = \max\{c(s,a), \epsilon\}$ with $\epsilon = \frac{S^2A}{K}$. % \todomout{maybe report the algorithm}

The main goal of this section is to empirically show that, despite the  $K^{2/3}$ regret bound when $c_{\min} = 0$, \UCSSP is competitive with \UCRLSSP whose regret bound scales as $\sqrt{K}$. We also show the role of the pivot horizon used by \UCSSP and of the two mentioned SSP planning approaches (\textcircled{a} and \textcircled{b}).


As done in the previous section, we start considering the uniform cost case. Fig.\,\ref{fig:bernstein.uniform}\emph{(left)} shows that \UCSSP outperforms \UCRLSSP using either planning \textcircled{a} or \textcircled{b}. From Fig.\,\ref{fig:bernstein.uniform}\emph{(right)} we can see that the lower regret of \UCSSP comes from the use of the pivot horizon. Indeed, when we integrate the pivot horizon idea in \UCRLSSP\footnote{\UCRLSSP uses the same condition of \UCRLB to terminate an algorithmic episode, i.e., when the number of visits to  a state-action pair is doubled, the algorithmic episode ends. When using the pivot horizon, we simply limit the number of steps in the algorithmic episode to be at most the pivot horizon (as done for \UCSSP). We also integrated the condition of planning every time the goal state is reached but we didn't observe any significant change in this domain.} the algorithms behave similarly.
In Fig.\,\ref{fig:bernstein.uniform}\emph{(right)} we can see that \UCRLSSP with \EVI~behaves as \UCRLB. This is due to the fact that SSP planning is equivalent to average reward planning in this setting (i.e., uniform cost). Furthermore, it shows that, in this domain, \UCRLSSP is not able to leverage the structure of the SSP problem. In contrast, \UCSSP adapts to the SSP problem thanks to the pivot horizon.

The second experiment focuses on the case when $c_{\min} =0$.
As shown in Fig.\,\ref{fig:bernstein.zero}\emph{(left)}, \UCSSP has a low regret even in this case.
\UCRLSSP achieves the same performance of \UCSSP only when using the pivot horizon as a stopping condition of the algorithmic episode.
This shows again that the stopping condition based on pivot horizon allows the algorithms to better adapt to the the SSP structure of this problem.
Finally, Fig.\,\ref{fig:bernstein.zero}\emph{(right)} shows that phase \ding{173} happens only at the early stages of the learning process. As a consequence, \UCSSP does not suffer additional regret due to phase \ding{173} in this domain.


\begin{figure}[tb]
  \centering
  \includegraphics[width=.48\textwidth]{./exp/bernstein/zero/regret_episodes.pdf}
  \includegraphics[width=.48\textwidth]{./exp/bernstein/zero/avglength_episodes.pdf}
  \caption{Evaluation of the algorithms with Bernstein inequalities and $c_{\min} = 0$. See Fig.\,\ref{fig:gridworld.zero} for details. For clarity, we report the planning technique used for each algorithm. We recall that \textcircled{a} stands for \EVI\ while \textcircled{b} stands for the two-step procedure (computing $\wt p$ and planning through value iteration). We use \textcolor{gray}{(orig.)} to denote the algorithm as described in the original paper. Right figure shows the average length of Phase \ding{172} and \ding{173} for \UCSSP with Bernstein inequalities and planning via \EVI.}
\label{fig:bernstein.zero}
\end{figure}

